The Spin Foam Approach to Quantum Gravity

This article reviews the present status of the spin foam approach to the quantization of gravity. Special attention is payed to the pedagogical presentation of the recently introduced new models for four dimensional quantum gravity. The models are motivated by a suitable implementation of the path integral quantization of the Plebanski formulation of gravity on a simplicial regularization. The article also includes a self-contained treatment of the 2+1 gravity. The simple nature of the latter provides the basis and a perspective for the analysis of both conceptual and technical issues that remain open in four dimensions.

==> coherent-states.tex <==
\subsection{Coherent states}

Let us first describe the coherent states for the
group ${\rm SU}(2)$. It will then be trivial to generalize
it to ${\rm SO}(4)$. 

We will start from the following obvious decomposition of the identity
operator in the representation space $V^j$ of dimension $\rd_j\equiv 2j+1$:
\be\label{ident-m}
1_j = \sum_m |j,m \rangle \langle j,m|,
\ee
where $|j,m\rangle, m\in[-j,j]$ is the usual orthonormal basis in $V^j$.
Let us rewrite the same operator by inserting in it the Kronecker delta
\be
\delta_{mm'} = \rd_j \int_{{\rm SU}(2)} dg \, t^j_{mj}(g) \overline{t^j_{m'j}(g)}
\ee
written in terms of an integral over the group. Here $t^j_{mj}(g)$ is the
matrix element of the group element $g$ in the representation $j$ computed between
the states $\langle j,m|$ and  $|j,j\rangle$, the latter being the highest weight state. More
generally:
\be
t^j_{mm'}(g) \equiv \langle j,m| g|j,m'\rangle.
\ee
This gives:
\be\label{ident-coherent}
1_j = \rd_j \sum_{mm'} |j,m \rangle \langle j,m'|
\int_{{\rm SU}(2)} dg \, t^j_{mj}(g) \overline{t^j_{m'j}(g)} =
\rd_j \int_{{\rm SU}(2)} dg \, |j,g \rangle \langle j,g|,
\ee
where we have introduced a notation:
\be\label{def}
|j,g \rangle \equiv g |j,j\rangle = \sum_m  |j,m \rangle t^j_{mj}(g) .
\ee
The states $|j,g \rangle$ are known as the coherent states, and
the last expression in (\ref{ident-coherent}) is the decomposition
of the identity in terms of these coherent states.


The decomposition of the identity (\ref{ident-coherent}) can be further simplified by 
noticing that the matrix elements $t^j_{mj}(g)$ and $t^j_{mj}(gh)$ differ only by a phase for 
any group element $h$ from the ${\rm U}(1)$ subgroup of ${\rm SU}(2)$. Therefore, the integral
in (\ref{ident-coherent}) can be taken over the coset $G/H, G={\rm SU}(2), H={\rm U}(1)$. Thus, we have:
\be
1_j = \rd_j \int_{G/H} dn \, |j,n \rangle \langle j,n|.
\ee
We will suppress the domain of integration $G/H$ in what follows.

The states $|j,n\rangle$ form (an over-complete) basis in $V^j$. 
One of the main motivations for using these states comes from the fact that they have  
a clear geometrical interpretation: Let $\hat{J}^{i}$ be the generators of the $SU(2)$ 
Lie algebra $[\hat{J}^{i},\hat{J}^{j}]= i \epsilon^{ijk} \hat{J}_{k}$. We can easily compute 
the expectation value of these generators in a given coherent state:
\be \label{geo}
X_{(j,n)}^i \sigma_i \equiv \langle j,n|\hat{J}^{i}|j,n \rangle \sigma_{i} =  j \, n\sigma_{3} n^{-1}
\equiv j \,n^{i} \sigma_{i},
\ee
where the quantities $\sigma_{i}$ are the Pauli matrices and 
we have denoted by the same letter the $SU(2)$ matrix $n$ that parametrized the coherent state 
and the three-dimensional unit vector $\vec{n}$ that this matrix corresponds to.
Thus we see that  $|j,n\rangle$ describes a vector in $\mathbb{R}^{3}$ of length $j$ and of direction 
determined by the action of $n$ on a unit reference vector. It is convenient to denote this vector by the 
same letter $\vec{n}$. This geometric interpretation will be extremely useful for us in what follows.

An important remark is as follows. Note that we could in principle define a notion of ``coherent'' state 
starting from any state $|j,m\rangle$ instead of the highest weight vector $|j,j\rangle$. Indeed, we
would have the same decomposition of unity as in (\ref{ident-coherent}). The geometrical interpretation would
be, however, drastically different. Namely, we could no longer interpret the states $g |j,m\rangle$ as representing
a vector lying on the sphere of radius $j$. Instead, these states correspond to a circle on this sphere of 
radius $\sqrt{j^{2}-m^{2}}$. Moreover, we can compute the dispersion of the quadratic operator $\hat{J}^{2}$ 
with the result being \be \Delta J^{2} = j + j^{2}-m^{2}.\ee
Thus, we see that only the highest and lowest states $m=\pm j$ lead to the coherent states that minimize the 
uncertainty relation.

It will be of crucial importance for us that there is not one but two coherent states $g |j,j\rangle\equiv |j,g\rangle$ and 
$g|j,-j\rangle\equiv \overline{|j,{g}\rangle}$. In order to relate them let us remark that the group element 
\be
\epsilon \equiv  \left( \begin{array}{cc} 0 & 1 \\ -1& 0 \end{array} \right)\ee
is such that 
\be 
g\epsilon = \epsilon \bar{g},
\ee
where $\bar{g}$ is the complex conjugate matrix.
The matrix element of $\epsilon$ in any representation is given by 
\be t_{nm}^{j}(\epsilon)= (-1)^{j-n} \delta_{n,-m}.\ee Thus, we have $\langle j,-j| \epsilon|j,j\rangle= (-1)^{2j}$ and therefore
the lowest weight vector can be obtained by the action of $\epsilon$ on $|j,j\rangle$. We have: 
\be
|j,-j\rangle = (-1)^{2j}\epsilon |j,j\rangle.
\ee 
More generally we can define the conjugate states
\be
\overline{|j,m\rangle} \equiv \epsilon |j,m\rangle = (-1)^{j+m}|j,-m\rangle.
\ee
These are called conjugate since their matrix elements are the complex 
conjugates of the usual matrix elements
\be 
\overline{\langle j,m|}g\overline{|j,n\rangle} = 
\langle j,m|\epsilon^{-1}g\epsilon{|j,n\rangle} = \overline{t_{mn}(g)} = (-1)^{2j+m+n}t_{ -m -n}(g)
\ee
We thus obtain two families of coherent states $|j,g\rangle$ and 
\be
\overline{|j,{g}\rangle} \equiv (-1)^{2j} g |j,-j\rangle =  \sum_m    \overline{|j,m \rangle} \overline{t^j_{mj}(g)}.
\ee

We are eventually interested in coherent states for ${\rm SO}(4)$. What this discussion shows is 
that one has four possible coherent states which are given by acting with an ${\rm SO}(4)$ group element 
on either of the following states: 
\be 
|j,j\rangle\otimes |j,j\rangle, \quad|j,j\rangle \otimes |j,-j\rangle, 
\quad|j,-j\rangle \otimes |j,j\rangle, \quad|j,-j\rangle \otimes |j,-j\rangle.
\ee
Note that these four states can be obtained from one another by the action of 
an $SO(4)$ group element. However, if one considers only the action of the diagonal $\SU(2)$ 
subgroup of elements of the form $(g,g)$ then there are two inequivalent 
states that cannot be related by such a transformation. As we will see below the state 
$|j,g\rangle\otimes |j,g\rangle$ will play the key role in the constructions of the topological sector 
whereas the state $|j,g\rangle\otimes \overline{|j,{g}\rangle}$ will be the one relevant to the gravitational sector.


==> groupaveraging.tex <==

\subsection{The path integral for generally covariant systems}
\label{valin}

LQG is based on the canonical (Hamiltonian) quantization of general relativity
whose gauge symmetry is diffeomorphism invariance. In the Hamiltonian
formulation the presence of gauge symmetries \cite{dirac} gives rise to
relationships among the phase space variables -- schematically $C(p,q)=0$ for
$(p,q)\in \Gamma$ -- which are referred to as \emph{constraints}. The
constraints restrict the set of possible states of the theory by requiring
them to lay on the constraint hyper-surface. In addition, through the Poisson
bracket, the constraints generate motion associated to gauge transformations on
the constraint surface (see Figure~\ref{phase}). The set of physical states
(the so called reduced phase space $\Gamma_{red}$) is isomorphic to the space
of orbits, i.e., two points on the same gauge orbit represent the same state in $\Gamma_{red}$
described in different gauges (Figure~\ref{phase}). 

In general relativity the absence of a preferred
notion of time implies that the Hamiltonian of gravity
is a linear combination of constraints. This means that Hamilton equations
cannot be interpreted as time evolution and rather correspond to motion along
gauge orbits of general relativity. In generally covariant systems conventional
time evolution is pure gauge: from an initial data satisfying the constraints
one recovers a spacetime by selecting a particular one-parameter family of
gauge-transformations (in the standard ADM context this amounts for choosing a
particular lapse function $N(t)$ and shift $N^a(t)$).
\begin{figure}[h]\!\!\!\!\!\!
\centerline{\hspace{0.5cm} \(
\begin{array}{c}
\includegraphics[height=5cm]{phase-space}
\end{array}\ \ \ \begin{array}{c}
\includegraphics[height=3cm]{quento}
\end{array}\) } \caption{On the left: the geometry of phase space in gauge
  theories. On the right: the quantization path of LQG (continuous arrows).}
\label{phase}
\end{figure}

From this perspective the notion of spacetime becomes secondary and
the dynamical interpretation of the the theory seems problematic (in
the quantum theory this is refered to as the \emph{``problem of
time''}).  A possible reason for this apparent problem is the central
role played by the spacetime representation of classical gravity
solutions.  However, the reason for this is to a large part due to the
applicability of the concept of \emph{test observers} (or more
generally \emph{test fields}) in classical general
relativity\epubtkFootnote{Most (if not all) of the textbook applications of
general relativity make use of this concept together with the
knowledge of certain exact solutions. In special situations there are
even preferred coordinate systems based on this notion which greatly simplify
interpretation (e.g.  co-moving observers in cosmology, or
observers at infinity for isolated systems).}. Due to the fact that
this idealization is a good approximation to the (classical) process
of observation the notion of spacetime is useful in classical gravity.


As emphasized by Einstein with his hole argument (see \cite{carlobook}
for a modern explanation) only the information in relational
statements (independent of any spacetime representation) have physical
meaning. In classical gravity it remains useful to have a spacetime
representation when dealing with idealized test observers. For
instance to solve the geodesic equation and then ask \emph{diff-invariant-questions} such as: {what is the proper time
elapsed on particle 1 between two succesive crossings with particle
2?}  However, already in the classical theory the advantage of the
spacetime picture becomes, by far, less clear if the test particles are
replaced by real objects coupling to the gravitational field
\epubtkFootnote{In this case one would need first to solve the constraints
of general relativity in order to find the initial data representing
the self-gravitating objects. Then one would have essentially two
choices: 1) Fix a lapse $N(t)$ and a shift $N^a(t)$, evolve with
the constraints, obtain a spacetime (out of the data) in a particular
gauge, and finally ask the \emph{diff-invariant-question}; or 2) try to
answer the question by simply studying the data itself (without
t-evolution). It is far from obvious whether the first option (the
conventional one) is any easier than the second.}.

However, this possibility is no longer available in quantum gravity
where at the Planck scale ($\ell_p\approx 10^{-33}\mathrm{\ cm}$) the quantum
fluctuations of the gravitational field become so important that there
is no way (not even in principle\epubtkFootnote{In order to make a Planck
scale observation we need a Planck energy probe (think of a Planck
energy photon). It would be absurd to suppose that one can disregard
the interaction of such photon with the gravitational field treating
it as test photon.}) to make observations without affecting the
gravitational field. In this context there cannot be any, \emph{a
priori}, notion of time and hence no notion of spacetime is possible at
the fundamental level. A spacetime picture would only arise in the
semi-classical regime with the identification of some subsystems that
approximate the notion of test observers.



What is the meaning of the path integral in the background
independent context? The previous discussion rules out the
conventional interpretation of the path integral. There is no meaningful
notion of transition amplitude between states at different times
$t_1>t_0$ or equivalently a notion of \emph{``unitary time
evolution''} represented by an operator $U(t_1-t_0)$.
Nevertheless, a path integral representation of generally
covariant systems arises as a tool for implementing the
constraints in the quantum theory as we argue below.

Due to the difficulty associated with the explicit description of the
reduced phase space $\Gamma_{\rm red}$, in LQG one follows Dirac's
prescription. One starts by quantizing unconstrained phase space
$\Gamma$, representing the canonical variables as self-adjoint
operators in a \emph{kinematical Hilbert space} $\Hk$. Poisson brackets
are replaced by commutators in the standard way, and the constraints
are promoted to self-adjoint operators (see Figure~\ref{phase}). If
there are no anomalies the Poisson algebra of classical constraints is
represented by the commutator algebra of the associated quantum constraints.  In
this way the quantum constraints become the infinitesimal generators
of gauge transformations in $\Hk$. The physical Hilbert space $\Hhp$ is
defineded as the kernel of the constraints, and hence to 
\emph{gauge invariant} states. Assuming for simplicity that there is
only one constraint we have \[\psi \in \Hhp\ \ \ {\rm iff}\ \ \
\exp[iN \hat C]|\psi\rangle=|\psi\rangle\ \ \
\forall \ \ \ N\in\R,\] where $U(N)=\exp[iN \hat C]$ is the unitary operator
associated to the gauge transformation generated by the constraint $C$ with
parameter $N$. One can characterize the set of gauge invariant states, and
hence construct $\Hhp$, by appropriately defining a notion of `averaging' along
the orbits generated by the constraints in $\Hk$. For instance if one can make
sense of the \emph{projector} \be P:\Hk \rightarrow \Hhp \ \ \ {\rm where } \ \ \
P:=\int dN\ U(N).\label{pipi}\ee It is apparent from the definition that for any $\psi\in
\Hk$ then $P\psi\in\Hhp$. The path integral representation arises in the
representation of the unitary operator $U(N)$ as a sum over \emph{gauge-histories} in a way which is technically analogous to standard path
integral in quantum mechanics. The physical interpretation is however quite
different as we will show in Section~\ref{gaugy}. The \emph{spin foam
representation} arises naturally as the path integral representation of the
field theoretical analog of $P$ in the context of LQG. Needles is to say that
many mathematical subtleties appear when one applies the above formal
construction to concrete examples (see \cite{marolf}).



==> modeloQM.tex <==
\subsection{A simple example: an isolated particle system}

Before going into the details of the definition of LQG we will
present the general ideas behind the quantization of generally
covariant systems using the simplest possible example: a non
relativistic isolated system. The dynamics in an isolated system is completely
encoded in an oriented curve in configuartion space up to parametrization: an orbit
(see Figure~\ref{barbour}). As in general relativity only relational
information encoded in such orbit is of dynamical content and there is no need
to the introduction of any external notion of time as long as the system stays
isolated. The equations of motion for an isolated system can be derived from
the following variational principle \cite{barb}:
\begin{equation}
S[\vec q_i]=\int d\lambda \sqrt{\left(E-V(\vec q_i)\right)\sum_{i=1}^N \frac{1}{2}m_i
\frac{d\vec q_i}{d\lambda} \cdot \frac{d\vec q_i}{d\lambda}}, \end{equation}
where $E$ is a constant characterizing the isolated system, $V$ is some
interaction potential among the $N$ particles with positions $\vec q_i$.
The previous action is obviously reparametrization invariant. Due to this
we expect the Hamiltonian of the theory to be weakly vanishing. More
precisely, the momenta $\vec p_i$ are given by
\begin{equation}
\vec p_i=\frac{\left(E-V(\vec q_i)\right) \frac{d\vec q_i}{d\lambda}}{\sqrt{\left(E-V(\vec q_i)\right)\sum_{i=1}^N \frac{1}{2}m_i
\frac{d\vec q_i}{d\lambda} \cdot \frac{d\vec q_i}{d\lambda}}},
\ee
from where one can check that they satisfy the constraint
\begin{equation}
C=\sum_{i=1}^N \frac{1}{2 m_i} \vec p_i\cdot \vec p_i+ V(\vec q_i)-E=0.
\ee
In other words, upon the customary Legendre transformation
the action takes the following Hamiltonian form
\begin{equation}
S(\vec q_i,\vec p_i, N)=\int d\lambda \sum_{i=1}^{N}\vec p_i  \frac{d\vec q_i}{d\lambda}  - N \left(\sum_{i=1}^N \frac{1}{2 m_i} \vec p_i\cdot \vec p_i+ V(\vec q_i)-E
\right).\end{equation}
The above action describes the Hamiltonian dynamics of an isolated system of
$N$ particles. No explicit time variable enters the formulation.

\epubtkImage{}{%
\begin{figure}[h!!!!!]
 \centerline{\includegraphics[height=4.5cm]{vela1}}
 \caption{At \textit{A} the candle has a certain length and the ball is at
   some position along a one dimensional line, at \textit{B} the candle has
   burned down to a shorter length and the ball is at a different
   place. An oriented curve in configuration space $\cal C$ encodes
   all the dynamical information of an isolated system. Physical
   motion is defined by the relationships between degrees of freedom
   at different points along the curve.}
\label{barbour}
\end{figure}}

Notice the formal similarity
with the action of general relativity (\ref{ADMA}) and
(\ref{TETA}). As in general relativity the Hamiltonian of the
system is zero on shell. This system is the simplest
example of generally covariant system.

Let us proceed and analyze the quantization of this action
according to the rules above.
\begin{itemize}

\item We first define an auxiliary or \emph{kinematical} Hilbert
space $\Hk$. In this case we can simply take $\Hk={\cal
L}^2(\R^N)$. Explicitly we use (kinematic) wave functions of
$\psi(\vec q_i)$ and define the inner product \begin{equation}
\label{fleme}<\phi,\psi>=\int \overline{\phi(\vec q_i)}
\psi(\vec q_i)  \prod_{i=1}^{N} d\vec q_i.\end{equation}
Promoting  the phase space variables to self adjoint
operators satisfying the appropriate commutation relations. In
this case the standard choice is that the $\vec q_i $ act simply by
multiplications and
$\vec
p_i=-i\hbar\partial/\partial \vec q_i$

\item The constraint becomes \begin{equation}\widehat
C=-\hbar^2\sum_{i=1}^N \frac{\partial^2}{\partial
\vec q_i \cdot \partial
\vec q_i}+ V(\vec q_i) - E. \end{equation} Notice that the constraint equation $\widehat
C|\psi>=0$ is nothing else than the familiar (time independent) Schr\"odinger equation.

\item The solutions of the quantum constraint are in this case
the solutions of the (time independent) Schroedinger equation.
The physical Hilbert space is therefore the subspace $\Hhp\subset {\cal
L}^2(\R^N)$ labelled by the eigenvalue $E$ of the standard
Hamiltonian---notice that this is a proper subspace only if $E$ is in the
discrete part of the spectrum of the Hamiltonian.

\item Dirac observables in this setting are those quantities that commute with
the standard Hamiltonian, i.e., those quantities that can be measured without
interference with the isolated nature of the system.
\end{itemize}

We have just reproduced standard quantum mechanics by quantizing
the reparametrization invariant formulation. As advertised in the general
framework of the Dirac program applied to generally covariant systems, the
full dynamics is contained in the quantum constraints -- here the
Schroedinger equation.


==> notas.tex <==

* Dans "Holomorphic Simplicity Constraints for 4d Spinfoam Models"
arXiv:1104.3683 avec MaitŽ, on a un peu conclu l'Žtude des contraintes
de simplicitŽ par le formalisme spinoriel (ou U(N)). On rŽ-Žcrit la
thŽorie BF en termes d'intertwiners cohŽrents et de spineurs et on
propose un nouveau modle de spinfoam rŽsolvant les nouvelles
contraintes de simplicitŽ (holomorphes). On montre que ces contraintes
holomorphes sont exactement Žquivalentes aux contraintes usuelles au
niveau classique. Au niveau quantique, on montre que l'on peut les
imposer fortement, que cela est Žquivalent ˆ une imposition faible
(comme EPRL) des contraintes quadratiques, et que le modele qui en
rŽsulte est piquŽ sur les amplitudes EPRL mais avec une Gaussienne (de
width fixe) autour des contraintes de simpmicitŽ diaogonales (les
irreps ne sont pas forcement gamma-simples, mais presque).
Un petit rŽsumŽ de ce boulot est en tant que proceeding de la loop
conference, si tu veux  jeter un tout petit coup d'oeil sans lire tout
le plus long papier, "Holomorphic Simplicity Constraints for 4d
Riemannian Spinfoam Models" arXiv:1111.1125.
Puis avec MaitŽ, Simone et Laurent, on a commencŽ a adapter ce
formalisme au cas Lorentzien, pour le moment juste au niveau
classique, "Holomorphic Lorentzian Simplicity Constraints"
arXiv:1107.5274

* Et plus rŽcemment dans "Classical Setting and Effective Dynamics for
Spinfoam Cosmology" arXiv:1111.2867 avec Merce, on a regardŽ en
dŽtails les calculs de spinfoam cosmology. D'une part, on peut dŽriver
exactement l'eq diff de la contrainte Wheeler-De Witt pour FRW
(modifiŽ) des amplitudes de spinfoam  (et non pas seulement dans la
limite a grand spin ou grand volume comme Carlo et Francesca), et
d'autre part on fait le lien explicite avec le cadre canonique et la
proposition d'un Hamiltonien sur le graph ˆ 2 vertex que j'avais fait
avec les espagnols d'aprs la proposition original de Carlo et
Francesca. On montre Žgalement comment prendre en compte la courbure
(et non la constante cosmolgique) et on explique les limites de cette
cosmologie FRW modifiŽe hors du cas plat.

Et biensur, si tu as le temps de jeter un coup d'oeil sur ces papiers,
tes commentaires/critiques/remarques sont les bienvenus!




I have read with great interest your latest review on the new spin
foam models, and I noticed that you are not aware of the important
results derived by myself and my collaborator M. Vojinovic last year,
concerning the semi-classical limit of spin foam models. We have shown
that the correct classical limit of a spin foam model can be obtained
if  the large-spin asymptotics of the vertex amplitude is of the
exp(iS) type, by using the effective action techniques, see

 1. arXiv:1110.6114 [pdf, ps, other]
   Title: Effective action for EPRL/FK spin foam models
   Authors: Aleksandar Mikovic, Marko Vojinovic
   Comments: v2: some changes in text, new references added; 4 pages,
proceedings
   of Loops  11 conference, Madrid; to appear in Journal of Physics:
Conference Series
   (JPCS)

and

2. arXiv:1104.1384 [pdf, ps, other]
   Title: Effective action and semiclassical limit of spin foam models
   Authors: A. Mikovic, M. Vojinovic
   Comments: Improved presentation, 2 references added. 15 pages, no figures
   Journal-ref: Class. Quant. Grav. 28, 225004 (2011)

This means that one has to redefine the EPRL-FK amplitude such that
the exponential asymptotics is achieved, since it was shown by Barrett
et al that this asymptotics is of the cosine type, i.e. W ~ N exp(iS)
+ M exp(-iS), where N and M are different from zero.This can be done
by an algebraic redefinition
                         W \to W + \sqrt{W - 4NM} ,
or by changing the f-coefficients in the linear combination of the
(15j)(15j') symbols, see
J. Engle, arxiv:1201.2187.

As far as the finiteness of a spin foam model is concerned, it depends
only on the scaling power lambda in the large-spin asimptotics of W,
and as shown in

   3. arXiv:1101.3294 [pdf, ps, other]
   Title: Finiteness of the EPRL/FK spin foam model
   Authors: Aleksandar Mikovic, Marko Vojinovic

there alwayas exists a real number p, independent of triangulation,
such that the rescaled vertex amplitude  W(j,i)/(\prod dim j )^p gives
a finite state sum.

==> report.tex <==

Report on `The spin foam approach to quantum gravity' by 
Alexandro Perez


This is an excellent review covering spin foams and related subjects. It discusses the essential technical points, reviews the status and points out the open problems in spin foam research. Also it is quite pedagogically written. I recommend it highly for publication.

The author may however consider the following points for corrections and improvements:

page 6:
'Gravitons would propagate respecting the causal structure of the unphysical background'.

%%This is not necessarily the case. Extracting fluctuating causal structures even in a perturbative approach has for instance been discussed in gr-qc/0610060 (Dittrich, Tambornino) or recently in 1111.7127 (Khavkine).

The references have been added in a footnote. Notice that the remark in the paper was about standard perturbative approaches. This has been clarified. Thanks for the remark.

page 2:
Here one could emphasize a bit more the importance of choosing the holonomy flux algebra as a starting point for quantization - many peculiar properties of LQG follow from this choice. (As the representation of this algebra is unique the choice of the observable algebra is the essential input.) Also that this choice is motivated by having an observable algebra which forms simple (diffeomorphism covariant) Poisson brackets.

This is a good point. Some text and an footnote has been added around eq. 6

page11:
Usage of 'anomaly free':  Here the term 'anomaly free' is ambigious. Thiemann's original Hamiltonian is anomaly free in the sense that the algebra between constraints is even Abelian. One could claim that this is not representing the actual hypersurface deformation algebra, hence anomalous in this sense. (On the other hand the algebra can only be evaluated on diffeomorphism invariant states, where the commutator would vanish.)

Nevertheless there are substantial doubts that the original Hamiltonian by Thiemann encodes the dynamics correctly, as the Abelian algebra is due to the ultra-local action of the operator. There are several other versions which are not ultra-local but then anomalous in the standard sense, i.e. the constraints become second class.

One could mention several alternatives that circumvent this problem, like the master constraint program, uniform discretization, or reduced phase quantization based on using matter fields as gauge fixings. Of course in all these approaches the question of the correct implementation of diffeomorphism symmetry remains open.

I DID NOT WANT TO GO INTO THE DETAILS HERE. MY STATEMENT IN THE ARTICLE IS CLEAR. I SAY THAT THE PROBLEM OF ANOMALIES REMAINS OPEN. 
I DO NOT CLAIM THAT THIEMANN'S PROPOSAL IS ANOMALY-FREE (I JUST SAY IS "WELL DEFINED"). 
I THINK HERE I AM IN AGREEMENT WITH THE REFEREE.  I JUST WANTED TO REMAIN VAGUE ON THIS COMPLICATED ISSUE.


page 17:
'Weak vs strong imposition of constraints': 
Also this is sometimes used as an argument that the BC model is not correct, I find that confusing. The BC model was defined without Immirzi parameter with a constraint algebra (of primary simplicity constraints), that is first class. 

THE QUANTUM CONSTRAINT ALGEBRA DOES NOT CLOSE (HENCE IS NOT FIRST CLASS)
THERE IS A MISLEADING ISSUE HERE DUE TO THE USE OF THE WORD "QUANTUM".
I HAVE ADDED THE FOOTNOTE: The six components $B^{IJ}$ are associated to invariant vector fields in the Lorentz group as a direct consequence of the discretization
procedure in spin foams. This makes them non commutative and render the simplicity constraints (functionals of the $B$ field alone) non commutative. The origin of the non commutativity of $B$ fields is similar to the non commutativity of fluxed in canonical LQG \cite{Ashtekar:1998ak}.

THE POINT IS THAT EVEN IN THE BC MODEL THE CONSTRAINTS (WRITTEN IN TERMS OF LEFT/RIGHT INVARIANT VECTORS FIELDS) ARE NON COMMUTATIVE.
IN ADDITION THE ALGEBRA DOES NOT CLOSE. WHICH MEANS THAT IF WE IMPOSE THEM STRONGLY WE ARE IMPOSING AND INFINITE SERIES OF CONSTRAINTS THAT FOLLOW FROM THE COMMUTATORS OF ARBITRARY ORDER. THIS IS TOO STRONG IN VIEW OF THE CLASSICAL THEORY.  

Hence it is quite correct to impose constraints 'strongly'. 

I HOPE I HAVE CLARIFIED THIS POINT

(The different versions of weak imposition of the constraints with the Immirzi parameter could however be described as rather non-standard. Later in the review it is mentioned that this has to be understood as semi-classical imposition.)

THIS IS A SPIN FOAM INPUT. IT IS NOT CLEAR WHAT A REASONABLE ALTERNATIVE WOULD BE AT THIS STAGE


page 26:
It is claimed that the LQG Hilbert space can be decomposed into a direct sum of orthogonal subspaces. The construction is rather a projective limit, which leads to non-trivial requirements (cylindrical consistency) on the structure (operators) of the theory. This point might lead to important differences if one considers for instance refining of graphs.

I AGREE WITH THE REFEREE. AGAIN HERE JUST WANTED TO PROVIDE THE BASIC IDEA ONLY. I HAVE NOW WRITEN
Roughly speaking \footnote{The construction is rather a projective limit ~\cite{ash3}.  This leads to non-trivial requirements (cylindrical consistency) on the structure (operators) of the theory. This point is very important for spin foams specially in considering the refining limit of amplitudes. We will revisit this issue in Section \label{}.},... AT THE BEGINNING OF THE CORRESPONDING SENTENCE. 

page 27:
`The fact that zero lies in the continuous spectrum of the diffeomorphism constraint'

The diffeomorphism constraint does not exist, only the finite group action does. 

I COMPLETELY AGREE. THIS WAS WRONG. I HAVE CORRECTED IT.

page 40:
-about divergencies and gauge fixing in BF: Here one could mention the recent work by Bonzom and Smerlak 1201.4996, indicating that complete gauge fixing might rather require the full simplicial complex instead of just the 2-complex.

THIS PAPER WAS NOT OUT AT THE TIME WHEN THE MANUSCRIPT WAS WRITTEN. THE FACT THAT ONE NEEDS THE FULL SIMPLICIAL COMPLEX WAS WELL KNOWN BEFORE THIS WORK. I HAVE ADDED THE REFERENCE.

page 45, eq (117) and the equ. before and also in equ (212)
There might be a typo: g_{ef} should rather be g_{ev} 

page 74: equ (211)

Here it might be useful to point out that the intertwiners appearing in (211) can be `integrated out' locally on each vertex/ simplex, different from the situation for EPRL or BF. Thus the BC does only depend on the 10 boundary spins as stated.

I AM NOT SURE WHAT IS THE REQUEST HERE.  THE FACT THAT WE LOOSE THE INTERTWINER QUANTUM NUMBER SEEM QUITE APPARENT IN OUR PRESENTATION.

p. 95, Sec. 14.8

Here one could refer to work on relational observables by Rovelli, Marolf, Dittrich, Marolf & Giddings & Hartle. 
For 4d gravity observables are expected to be rather non-local. Additionally for discrete theories diffeomorphism invariant observables should not refer to any fixed vertex or edge etc. of the underlying simplicial complex.  These are certainly not relational in nature. (The n-point functions so far used in spin foams do not satisfy this requirement.)

I AGREE COMPLETELY WITH THE STATEMENT PART OF THE ABOVE COMMENT. FOR THE REFERENCES I WOULD BE GRATEFUL IF THE REFEREE WOULD BE MORE CONCRETE. I WILL BE HAPPY TO CONSIDER/ADDING THEM.

Sec. 14.9

One could add to this discussion that the view that spin foams represent diffeomorphism equivalence classes of geometries is incompatible with the idea that spin foams should act as a projector onto the solutions of constraints. A path integral would only act as a projector if it includes gauge symmetries. Also one would expect the solutions to be outside the Hilbert space that is non-normalizable. That is the path integral should lead to (gauge) divergencies -- which implement the projector. 

YES, I DO AGREE. I HAVE ADDED A COMMENT. HOWEVER, I DO NOT AGREE WITH VERY THE LAST SENTENCE. IN 3D (AS WE DO IT KARIM NOUI AND I) ONE DOES NOT HAVE DIVERGENCES IN TRANSITION AMPLITUDES YET ONE GETS A PROJECTOR. BUT OF COURS PHYSICAL STATES HAVE INFINITE KINEMATICAL NORM. IF THAT IS WHAT THE REFEREE MEANS BY THE LAST SENTENCE WE DO AGREE.

Sec 14.10

Discretization independence is not only a problem of spin foams but also of Regge gravity. Even linearized classical Regge calculus is not discretization independent in 4d as shown in Dittrich, Steinhaus 1110.6866, but also the question of a triangulation independent/ anomaly free measure is discussed there.

One could mention that discretization independence is connected to the issue of diffeomorphism symmetry as discussed in Sec. 14. 9. There is evidence [40,43, 1201.3840] that implementation of diffeomorphism symmetry into the models will lead to discretization independence. The reason is that both problems can be solved by constructing the perfect action, which as a fixed point action is invariant under change of triangulation.

I HAVE ADDED SOME TEXT AND REFERENCES AT THE END OF 14.10

Also the question is raised whether the amplitudes remain finite under coarse graining/ in the continuum limit. As mentioned before, if spin foams are expected to act as projector onto solutions of the constraints one should expect at least divergencies due to integration over gauge orbits.

THESE SHOULD BE APPROPRIATELY GAUGE FIXED IF WE TAKE SERIOUSLY THE LESSONS FROM 3D (NOUI-PEREZ)
BUT THIS IS A QUESTION THAT WE COULD DISCUSS FURTHER OUTSIDE THIS ANONYMOUS EXCHANGE.





==> topoinvarianceBF.tex <==
\section{Topological invariance in BF-theory}
\label{chp:topo}

In this appendix we show the discretization independence of the
path integral introduced in Chapter~\ref{chp:bf} of BF theory defined in terms of a compact group $G$. 
For simplicity we will consider the lower-dimensional cases $d \le 4$, but the general scheme 
presented here can be extended to arbitrary dimensions. The proofs presented are rather
formal due to the existence of divergences (recall previous discussions about
bubble divergences). A rigorous statement about topological invariance (triangulation invariance) 
of ${\cal Z}_{BF}$ can be
made if a suitable regularization is introduced. 
This has been done in terms of a quantum deformation of the group
(for the deformation parameter $q$ a root of unity) in 
 \cite{turaev-viro} and  \cite{CraneYetter} for BF theory in three and four dimensions, respectively.
The techniques presented here can be straightforwardly generalized to quantum groups \cite{ro}.
The applications of these techniques are independent of the particular combinatorics of triangulations, which
allows us to prove the stronger result of invariance under arbitrary discretization of the manifold
represented by an arbitrary cellular decomposition of $\cal M$. For a rigorous proof of the results presented here in the
regularized case see reference  \cite{raf}. 


\subsection{General identities in representation theory}
\label{ident}

We start by reviewing some general properties of representation theory. Here we also introduce 
a graphical notation which allow us to give a remarkably simple proof of topological invariance 
of BF theory in the following sections. 

In Chapter {\ref{chp:bf}} we used certain formulas for the integration of the tensor product 
of two, three, and four representation matrices on the group (see equations (\ref{orto}),(\ref{3dp}), and (\ref{4dp})).
Let us prove these identities for a general number, say $n$, of representation matrices in the integrand.
In order to do so we expand our tensor product $\rho_1 \otimes \rho_2 \dots \otimes \rho_n$ into irreducible representations, namely
\begin{equation}
\rho_1 \otimes \rho_2 \dots \otimes \rho_n = \bigoplus \limits_{\rho^{\prime}} \rho^{\prime},
\end{equation}
where in general the first term on the right corresponds to the trivial representation.
One of the basic properties of the integration corresponds to the fact that the integral of a single
representation is zero unless it corresponds to the trivial representation, i.e., $\int dg \rho(g)= \delta_{\rho_0}$.
Integrating both sides of the previous equation we obtain
\begin{equation}\label{cable0}
\int dg \rho_1(g) \otimes \rho_2(g) \dots \otimes \rho_n(g)= \ {\rm projector \ into \ the \ trivial \ representation},
\end{equation}
where the fact that this is a projection comes from the invariance and normalization of the Haar measure (one can easily check that the LHS squared equals itself). Finally, if we choose an orthonormal basis of invariant vectors 
$\{ C^{\va \iota}_{\va \rho_1 \dots \rho_n} \}$ in $\rho_1 \otimes \rho_2 \dots \otimes \rho_n$ the projector becomes
\begin{equation}\label{kable}
\int dg \rho_1(g) \otimes \rho_2(g) \dots \otimes \rho_n(g)= \sum_{\iota} C^{\va \iota}_{\va \rho_1 \dots \rho_n} \ 
C^{*{\va \iota}}_{\va \rho_1 \dots \rho_n},
\end{equation}
where $\iota$ labels the basis elements. 

It is convenient to introduce a graphical
notation for equation (\ref{cable0}). We represent irreducible representation matrices by lines that we call 
wires. The tensor product of representations is given by a set of parallel wires labeled by the corresponding 
representations. We represent the  projector into the trivial component of the tensor product of irreducible 
representations by a dark rectangle which we call a {\em cable}. In terms of this notation equation (\ref{cable0})
becomes
\begin{equation}\label{cable}
\int dg \rho_1(g) \otimes \dots \otimes \rho_n(g)= \begin{array}{c} 
\includegraphics[width=1.3cm]{cable}\end{array}.
\end{equation}
Cables satisfy identities that can be easily translated into graphical operations.
These identities can be used to prove the discretization invariance of the BF state sum models presented in 
Chapter \ref{chp:bf}. For example, the fact that the cable correspond to a projection is 
graphically represented by the following equation:
\begin{equation}
\begin{array}{c} 
\includegraphics[width=.9cm]{gauge}\end{array} = \begin{array}{c} 
\includegraphics[width=.9cm]{gaugea}\end{array},
\end{equation}
where we have written the identity for the tensor product of three irreducible representations,
i.e. three wires. The same identity holds for any number of wires. Another property of cables is that 
for certain wire-cable configurations some of the cables might be redundant, i.e., they can be dropped
without changing the value of the diagram. This property is a consequence of the $G$ gauge 
invariance of BF theory. The corresponding general identity is
\begin{equation}\label{ggene}
\begin{array}{c} 
\includegraphics[width=2.5cm]{GG}\end{array} = \begin{array}{c} 
\includegraphics[width=2.5cm]{GGa}\end{array},
\end{equation}
where the dotted box denotes any cable-wire diagram, and the number of external cables is arbitrary
as well as the number of wires in each individual cable. The identity reads as follows: if in a planar projection
of an arbitrary configuration of wires and cables we can find a closed loop which cuts only cables then one of the
corresponding cables is redundant and can be removed. One can easily prove the previous general identity in a completely
algebraic way  \cite{ro,raf}.  
In order not to introduce new notation and technicalities we do not prove the previous equation here.
We will simply show its validity in some particular cases of interest.
A specially simple case of equation (\ref{ggene}) is   
\begin{equation}\label{tdt}
\begin{array}{c} 
\includegraphics[width=1.3cm]{gauge1}\end{array} = \begin{array}{c} 
\includegraphics[width=1.3cm]{gauge1a}\end{array}.
\end{equation}
Lets prove the previous equation by writing the LHS explicitly. Putting in indices and choosing the 
representations for which the diagram is nonvanishing we obtain
\begin{eqnarray}
&& \nonumber \int dg_1\ {\rho_1(g_1)}_{ab} {\rho_2(g_1)}_{cd}
\int dg_2\
 {\rho_1(g_2)}_{be}{\rho_3(g_2)}_{fg} 
\int dg_1\ {\rho^*_3(g_3)}_{fh}{\rho_2(g_3)}_{dj}=\\
&& \nonumber \int dg_1dg_2dg_3\ {\rho_1(g_1g_2)}_{ae} {\rho_2(g_1g_3)}_{cj}
 {\rho_3(g_2g^{-1}_3)}_{fh}=\\
&&\int d\gamma_2d\gamma_3\ {\rho_1(\gamma_2)}_{ae} {\rho_2(\gamma_3)}_{cj}
 {\rho_3(\gamma_2\gamma^{-1}_3)}_{fh},
\end{eqnarray}
where in the first line repeated indices are summed over and in the last line we have
used the normalization and invariance of the Haar measure to obtain the RHS of (\ref{tdt})
after introducing the new integration variables $\gamma_2=g_1g_2$ and $\gamma_3=g_1g_3$.
A similar computation shows that
\begin{equation}\label{tres}
\begin{array}{c} 
\includegraphics[width=1.7cm]{gauge2}\end{array} = \begin{array}{c} 
\includegraphics[width=1.7cm]{gauge2a}\end{array},
\end{equation}
and
\begin{equation}\label{cuatro}
\begin{array}{c} 
\includegraphics[width=2.3cm]{gauge3}\end{array} = \begin{array}{c} 
\includegraphics[width=2.3cm]{gauge3a}\end{array}.
\end{equation}
As we mentioned above, a proof of the general identity (\ref{ggene}) can be given
using a completely algebraic approach. 

There is another identity which is fundamental in what follows, namely
\begin{eqnarray}\label{pito}
\sum \limits_k \Delta_k \begin{array}{c} 
\includegraphics[width=1.75cm]{ident1}\end{array}=\begin{array}{c} 
\includegraphics[width=.99cm]{ident2}\end{array},
\end{eqnarray}
where $\Delta_k$ is the dimension of the representation $k$.
According to our notation, the integrand 
corresponding to the cable on LHS of the previous equation is given by the tensor product 
$k \otimes \rho_1 \otimes \dots \otimes \rho_n$.
In order to prove (\ref{pito}) we expand the tensor product $\rho_1 \otimes \dots \otimes \rho_n$  in terms of a direct
sum of irreducible representations, namely
\begin{equation}\label{kiri}
\rho_1 \otimes \dots \otimes \rho_n=\rho^{(0)} \oplus \rho^{(1)} \oplus \dots \oplus \rho^{(j)},
\end{equation}
for some $j \in \N$. Now the integrand on the LHS of (\ref{pito}) becomes a direct sum of terms of the
form $k \otimes \rho^{(i)}$, i.e., of tensor products of only two representations. We can then apply the
orthonormality of representations (already introduced in Chapter (\ref{chp:bf})), which corresponds to the 
simplest case of equation (\ref{kable}). In this notation it becomes 
\begin{eqnarray}\label{qiri}
\begin{array}{c} 
\includegraphics[width=1.4cm]{ident01}\end{array}=\delta_{k \rho}\frac 1 {\Delta_\rho} \begin{array}{c} 
\includegraphics[width=1.cm]{ident02}\end{array},
\end{eqnarray}
where the factor $\Delta_\rho$ in the denominator normalizes the corresponding intertwiners.
After applying the previous equation we recover precisely $\rho_1 \otimes \dots \otimes \rho_n$ as in (\ref{kiri}) which
corresponds to the RHS of identity (\ref{pito}).

The last important identity we will use in the sequel is
\begin{equation}\label{martin}
\sum \limits_{k} \Delta_{k}
\begin{array}{c} 
\includegraphics[width=2.cm]{martin}\end{array} = \begin{array}{c} 
\includegraphics[width=1.1cm]{martin1}\end{array}.
\end{equation}
The proof follows the same path as with the previous identity. We start
with the RHS. Assume that the labeling of the wires in the cable on the left
is $\rho_1 \otimes \dots \otimes \rho_n \otimes k$. Now expand the 
tensor product $\rho_1 \otimes \dots \otimes \rho_n$  in terms of a direct
sum of irreducible representations as in (\ref{kiri}). The left cable 
becomes a direct sum of cables with only two wires ($k \otimes \rho^{(i)}$). 
We can apply (\ref{qiri}) to each individual term in the direct sum which inserts the
given representation $\rho^{(i)}$ into the cable on the right on the RHS of the equation. 
Therefore, we obtain a direct sum of single cables where the first wire is labeled 
by $\rho^{(i)}$ which, using (\ref{kiri}), yields the RHS of equation (\ref{martin}).

Why is this notation relevant for the study of the state sum models of BF theory?
The answer is in the fact that the partition function of BF theory corresponds to 
the evaluation of a particular cable-wires diagram. Recall that according to the definition
of the path integration for BF theory in Chapter \ref{chp:bf}, the partition function is given by
(see equation (\ref{coloring}))
\begin{equation}\label{vanino}
{\cal Z}(\Delta)=\sum \limits_{ {\cal C}:\{f\} \rightarrow \{ {\rm irrep}(G)\} }  
\ \prod_{f \in {\cal J}_{\va \Delta}} 
\Delta_{\rho_f}  \int \ \prod_{e \in {\cal J}_{\va \Delta}} 
dg_e  \ {\rm Tr}\left[\rho_f(g^1_e\dots g^{\va N}_e)\right].
\end{equation}
Expanding ${\rm Tr}\left[\rho_f(g^1_e\dots g^{\va N}_e)\right]$ and collecting terms
corresponding to the same group element $g_e$ we notice that there will be a $k$-wired
cable for each edge in ${\cal J}_{\va \Delta}$, where $k=d$ for $d$ the dimension of the
manifold. The wires are connected such that every closed loop corresponds to a face 
$f \in {\cal J}_{\va \Delta}$. Equations (\ref{pito}) and the gauge-fixing identity (\ref{ggene})
will allow us to go from a discretization to another corresponding to the same manifold $\cal M$.
The moves that control this process are known as Pachner moves whose definition is given in the next 
section.

\subsection{Pachner moves}\label{Pach}

Consider an $(n+1)$-dimensional simplex $s^{(n+1)}$. Let $\alpha =\partial
s^{(n+1)}$ be its boundary. $\alpha$ is naturally a compact triangulated 
$n$-dimensional manifold, formed by $n+2$ $n$-simplices $s^{(n)}_{1},\ldots,
s^{(n)}_{n+2}$. Let $m$ be $1\le m\le n+1$. Pick $m$ of the $n+2$ $n$-simplices
on $\alpha$, and denote them as ``past'' simplices. Denote the remaining $n+2-m$
as the ``future'' simplices. Notice that since all the $s^{(n)}_{i}$ are
contiguous to each other, $\alpha$ gets divided in this way in two regions:
the past region, formed by the $m$ past simplices, and the future region,
formed by the $n+2-m$ ones. The past region and the future region are two 
$n$-dimensional triangulated manifolds sharing the same boundary. A 
($(n+1)$-dimensional) $(m,(n+2-m))$ Pachner move is defined as the replacement of a
past region formed by $m$ $n$-simplices, with the corresponding future region,
formed by $(n+2-m)$ $n$-simplices. Clearly, an $(i,j)$ Pachner move is the
inverse of a $(j,i)$ Pachner move. One can prove that any two triangulations 
$\Delta$ and $\Delta^{\prime}$ of an $n$-dimensional manifold are connected
by sequences of Pachner moves \cite{udo}.

Let us give a few examples that might be illuminating. Let us start
with n=2. In this case, $s^{(n+1)}$ is a tetrahedron. Its boundary is formed
by four triangles. Consider the $(1,3)$ Pachner move. That is, consider one of
the four triangles of the tetrahedron as the past, and the other three as the
future. Notice that the boundary of the past is the same as the boundary of
the future. The $(1,3)$ Pachner move is thus the replacement of a triangle
with three triangles. This move is shown on the left of Figure~\ref{trito},
while the $(2,2)$ move is shown on the right. 
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{tritoa}\ \ \ \ \ \ \ \ \ \ \ \ \ \  
\includegraphics[width=5cm]{tritob}}    
\caption{Pachner moves in two dimensions.}\label{trito}
\end{figure}
 
In three dimensions there are two possible Pachner moves -- the $(1,4)$ Pachner 
move and the $(2,4)$ Pachner move -- plus their inverses.  
In the $(1,4)$ one creates four tetrahedra out of one in the following way:
put a point $p$ in the interior of the original tetrahedron whose vertices are
labeled $p_i, \ i=1,\dots 4$, and add the four $1$-simplexes $(p,p_{i})$,
the six triangles $(p,p_{i},p_{j})$, and the four tetrahedra $(p,p_{i},p_{j},p_{k})$
(where $i \ne j \ne k \ne l$).

The $(2,4)$ Pachner move consists of the splitting of two 
tetrahedra into three tetrahedra. One replaces two tetrahedra $(u,p_1,p_2,p_3)$, and 
$(d,p_1,p_2,p_3)$ ($u,d$ for `up' and `down' ), sharing the triangle $(p_1,p_2,p_3)$ with the 
three tetrahedra $(u,d,p_{i},p_{j})$ where $i\ne j =1,\ldots 3$. 
 
In four dimensions there are 3 possible Pachner moves --the 1-5, the
2-4, and the 3-3 Pachner moves respectively-- plus their inverses. 
In terms of a 4d triangulation, the 1-5 move is defined by the split 
of a 4-simplex into five 4-simplices.  More precisely, we 
put a point $p$ in the interior of the 4-simplex with vertices $p_{i}, 
i=1,\ldots 5$, and we add the five segments $(p,p_{i})$, the ten triangles 
$(p,p_{i},p_{j})$, the ten tetrahedra $(p,p_{i},p_{j},p_{k})$, and the 
five 4-simplices $(p,p_{i},p_{j},p_{k},p_{l})$ (where $i \ne j \ne k \ne l$). 

In the 2-4 move, we replace  the two 4-simplexes  $(u,p_1,p_2,p_3,p_4)$, and 
$(d,p_1,p_2,p_3,p_4)$, sharing the tetrahedron $(p_1,p_2,p_3,p_4)$ with the 
four 4-simplices $(u,d,p_{i},p_{j},p_{k})$ where $i\ne j\ne k=1,\ldots 4$. 

In the $(3,3)$ Pachner move one rearranges three 4-simplexes into three new ones.
One starts with three 4-simplexes $(a,b,p_1,p_2,p_3)$, $(b,c,p_1,p_2,p_3)$ and
$(c,a,p_1,p_2,p_3)$ sharing the triangle $(p_1,p_2,p_3)$, and one defines the three
new 4-simplexes $(p_1,p_2,a,b,c)$, $(p_2,p_3,a,b,c)$, and $(p_3,p_1,a,b,c)$.

The series of Pachner moves described above can be translated in terms of 
the corresponding moves in the dual $2$-complex ${\cal J}_{\Delta}$. These moves
are the relevant ones for the topological invariance proof of the BF partition function, since
as was discussed in Chapter (\ref{chp:bf}), given a triangulation $\Delta$ of $\cal M$,
the partition function is defined on the dual $2$-complex ${\cal J}_{\Delta}$. 
As mentioned above, it can be shown that any two triangulations $\Delta$ and
$\Delta^{\prime}$ of the manifold $\cal M$ are related by a series of Pachner moves.
Consequently, there is a sequence of Pachner moves connecting ${\cal J}_{\Delta}$ to
${\cal J}_{\Delta^{\prime}}$. The idea in proving triangulation invariance of ${\cal Z}_{BF}$
is to show that it is invariant under individual Pachner moves and therefore under
any arbitrary correspondent sequence. 

\section{Triangulation independence of the BF path integration}

In this section we prove the triangulation independence of the state sum formulae for
quantum BF theory presented in Chapter (\ref{chp:bf}), equation (\ref{tinv}). The proofs
given here should be regarded as formal from the mathematical point of view since we
will be manipulating with a certain infinite factors in the argumentation. This is because
of the presence of the noncompact gauge freedom (\ref{gauge2}) in BF theory which induces infinite contributions
in the path integral formula every time there is a closed bubble in ${\cal J}_{\va \Delta}$. 
These infinities are rather trivial from the physical point of view
and can be eliminated by the standard Faddeev-Popov procedure of dividing by the volume of the gauge group 
\cite{freidel2}. 
As we mentioned before, another regularization consists of working with certain quantum deformation of
the gauge group which essentially introduces a cutoff in momentum space regularizing the partition function.
In this context a rigorous proof of triangulation independence can be given. In the $2$-dimensional
case this fact is trivial from the form of the partition function (\ref{genus}). In three and
four dimensions the invariance of the regularized partition function is proven in  \cite{turaev-viro} and  \cite{CraneYetter1}, respectively. 

In this section we introduce a new technique for proving invariance that differs from the one of  \cite{turaev-viro,CraneYetter1} based on the Biederharn-Elliot identities satisfied by $3Nj$-symbols \cite{naranja}. These identities are only useful
in the context of triangulations. The new tools are 
rather powerful and allow us to go beyond the combinatorics of triangulations to define the
problem of invariance under an ``arbitrary'' discretization (represented by an arbitrary cellular decomposition of the manifold) without any additional effort. This is sketched in the last subsection. 
The new techniques are illustrated at the level of the classical group and therefore
we have to deal with infinite factors. However, a regularized version
of these proofs equivalent to the ones given in  \cite{turaev-viro,CraneYetter1} as well as the 
extention of the results to general cellular complex can be found in  \cite{raf}.  


\subsection{Triangulation independence of ${\cal Z}_{BF}$ in 3 dimensions.}
 
\subsubsection{The $(4,1)$ move}

We start by showing invariance of the $3d$ BF partition function under the $(4,1)$ Pachner move. 
So, we start with the four-tetrahedra diagram described above. In terms of cables and wires the
diagram is shown on the left in Figure~{\ref{fig:1}}. We want to arrive to the $1$-tetrahedron 
diagram shown on the right
of Figure~{\ref{figg:3}} using the graphical identities proven above. The first step is to apply the
gauge-fixing identity (\ref{tres}) to eliminate redundant cables from the 4-tetrahedra diagram. The
result of one of the possible ways of doing that is shown on the right of Figure~{\ref{fig:1}}.
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM3d31a} 
\includegraphics[width=5cm]{PM3d31b}}    
\caption{The diagram on the left shows the dual 2-complex corresponding to a
piece of the triangulation $\Delta$ consisting of four tetrahedra interconnected
as described above in the description of the $(1-4)$ Pachner move. On the right the gauge-fixing
identity (\ref{tres}) has been applied.}\label{fig:1}
\end{figure}
Now we can continue to eliminate internal cables implementing equation (\ref{pito}) on the emphasized 
cable on the same diagram. Notice that the factor $\Delta_{\rho}$ in (\ref{pito}) and the corresponding sum over representations is provided by the form of the partition function (\ref{vanino}).
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM3d31c} 
\includegraphics[width=5cm]{PM3d31d}}    
\caption{Elimination of the remaining internal cables applying equation (\ref{pito}).}\label{fig:2}
\end{figure}
All the internal cables can be eliminated applying equation (\ref{pito}).
At the end of this process we obtain the $1$-tetrahedron diagram with an additional
closed wire loop. Such a closed loop corresponds to the trace of the identity in the
corresponding representation, i.e., $\Delta_{\rho}$, which together with the factor
$\Delta_{\rho}$ in (\ref{vanino}) gives an overall factor $\tau=\sum_{\rho} \Delta^2_{\rho}$.
As we discussed in Chapter (\ref{chp:bf}) this divergent factor is associated to the noncompact
gauge symmetry $B \rightarrow B+d_{\va A} \eta$ (see Chapter (\ref{chp:bf})) of BF theory, 
and should correspondingly be divided out of the partition function according to the 
standard Faddeev-Popov procedure \cite{FP}. This makes the partition function invariant under
the $(1,4)$ move, since the relevant quantity is now
\begin{equation}\label{moco}
{\cal Z}^{\prime}_{BF}=\tau^{-n^{\va (3)}_b}{\cal Z}_{BF},
\end{equation}
where $n^{\va (3)}_b$ is the number of bubbles in the dual 2-complex ${\cal J}_{\Delta}$. By dualization,
this number corresponds to the number of vertices in the triangulation $\Delta$ 
denoted $v_{\va \Delta}$ in Chapter \ref{chp:bf}.
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM3d31e} 
\includegraphics[width=5cm]{PM3d31}}    
\caption{Once the last internal cable is eliminated we end up with a closed wire contributing to 
the amplitude with a factor $\tau=\sum_{\rho} \Delta^2_{\rho}$. The remaining diagram corresponds precisely
to the dual of a tetrahedron.}\label{figg:3}
\end{figure}

\subsubsection{The $(3,2)$ move}

Using the same techniques we can prove invariance of ${\cal Z}^{\prime}_{BF}$
under the $(3,2)$ Pachner move and complete in this way the proof of triangulation invariance of
the BF path integral in three dimensions. So, we start with the diagram on the left of Figure~{\ref{fig:4}}
representing the 3-tetrahedra appearing in the $(3,2)$ Pachner move in the dual cable-wire diagrammatic way
(see (\ref{Pach})). We gauge fix two of the cables using (\ref{tres}) and eliminate the last internal cable
by means of (\ref{pito}) (left diagram in Figure~{\ref{figg:5}}). 
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM3d32a} 
\includegraphics[width=5cm]{PM3d32c}}    
\caption{The 3-2 Pachner move: starting with the diagram on the left
we gauge fix and then make use of equation (\ref{pito}) once.}\label{fig:4}
\end{figure}
The evaluation of a cable-wire diagram depends only on the combinatorics of
the connections; therefore, the value does not change if we deform a diagram
without changing the way wires are connected to each other. On the left of 
Figure~{\ref{figg:5}} we have deformed the previous diagram. On the right, we add a redundant
cable using (\ref{tres}) to obtain finally the sought for $2$-tetrahedra diagram.
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=3.6cm]{PM3d32} 
\includegraphics[width=3.6cm]{PM3d32d}}    
\caption{The evaluation of the partition function depends only on 
the combinatorics of the wiring (it only matters what is connected to what).
We obtain the diagram on left by continuously deforming the 
the previous graph. Finally, we obtain the cable-wire diagram corresponding to
two tetrahedra sharing a triangle by adding a redundant cable (using (\ref{tres})). }\label{figg:5}
\end{figure}
%\begin{figure}[h]
%\centerline{\hspace{0.5cm} 
%\includegraphics[width=4.5cm]{PM3d32d}}    
%\end{figure}
We have shown that the partition function ${\cal Z}^{\prime}_{BF}$ in (\ref{moco}) is a topological invariant,
which proves the statement we made in Chapter (\ref{chp:bf}) in equation (\ref{tinv}) for 
$\alpha=\tau^{n^{\va (3)}_b-n^{{\va (3)}\prime}_b}$.


\subsection{Triangulation independence of ${\cal Z}_{BF}$ in 4 dimensions.}

In four dimensions the proof is equivalent to the three-dimensional case.
The combinatorics changes, cables have four wires, and the relevant gauge-fixing identity
is now equation (\ref{cuatro}).  

\subsubsection{The $(1,5)$ Pachner move}

We start with the five 4-simplex cable-wire diagram on the left of Figure~{\ref{fig:6}}
corresponding to the configuration described above in (\ref{Pach}). We eliminate four internal redundant
cables using (\ref{cuatro}), and the six remaining ones using (\ref{pito}) (see Figure~{\ref{fig:7}}).
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=7cm]{PM4d51} 
\includegraphics[width=7cm]{PM4d51a}} 
\caption{The $(5,1)$ Pachner move. One gauge fixes four of the internal
cables using identity (\ref{cuatro}), the remaining internal cables can be removed using
(\ref{pito}).} \label{fig:6}  
\end{figure}
%\begin{figure}[h]
%\centerline{\hspace{0.5cm} 
%\includegraphics[width=3cm]{PM4d51b} 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,
%\includegraphics[width=3cm]{PM4d51c}}    
%\end{figure}
%\begin{figure}[h]
%\centerline{\hspace{0.5cm} 
%\includegraphics[width=3cm]{PM4d51d} 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,
%\includegraphics[width=3cm]{PM4d51e}}    
%\end{figure}
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=7cm]{PM4d51c} 
\includegraphics[width=7cm]{PM4d51g}}
\caption{One goes from the diagram on the right to the one on the
left by means of the repeated use of equation (\ref{pito}). Four closed wires remain
on the right, so one obtains the one 4-simples cable-wire diagram times $\tau^4$.}\label{fig:7}
\end{figure}
After this sequence of applications of (\ref{pito}) we obtain the corresponding one 4-simplex
diagram shown on the right of Figure~{\ref{fig:7}} plus four additional closed loops which contribute as 
a $\tau^4$ factor. As in three dimensions, if we denote by $n^{\va (4)}_b$ and $n^{\va (3)}_b$
the number of 4-bubbles and 3-bubbles respectively the rescaled partition function
\begin{equation}\label{topete}
{\cal Z}^{\prime}_{BF}=\tau^{n^{\va (4)}_b-n^{\va (3)}_b}{\cal Z}_{BF}
\end{equation}
is the appropriate invariant quantity. On the left of Figure~{\ref{fig:6}} 
the set of ten internal cables with the corresponding wires connected in such a way as to define
ten internal faces, define the one 4-bubble contained in the diagram. Each sub-diagram defined by
taking only four vertices defines a tetrahedron-like 3-bubble; there are five such bubbles,
so $n^{\va (4)}_b-n^{\va (3)}_b$ equals 4.
In the final stage (right diagram in Figure~{\ref{fig:7}}) there are no remaining bubbles; therefore,
the factor $\tau^4$ compensates the change in $n^{\va (4)}_b-n^{\va (3)}_b$ in order to leave
(\ref{topete}) invariant.

\subsubsection{The $(4,2)$ move}

The $(4,2)$ Pachner move can be implemented using the same techniques as above.
The process is illustrated in Figures~{\ref{fig:8}} and {\ref{fig:9}}. In the initial four 4-simplex
configuration there is a single (tetrahedron-like) 3-bubble defined by the six internal cables and the four 
corresponding faces.  
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM4d42a} 
\includegraphics[width=5cm]{PM4d42b}}    
\caption{On the left, the four 4-simplex configuration intervening in the $(4,2)$ Pachner move.
As in the previous case we eliminate internal cables using identities (\ref{cuatro}) and (\ref{pito}).}\label{fig:8}
\end{figure}
%\begin{figure}[h]
%\centerline{\hspace{0.5cm} 
%\includegraphics[width=3cm]{PM4d42c} 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,
%\includegraphics[width=3cm]{PM4d42d}}    
%\end{figure}
In the final two 4-simplex configuration no bubbles remain.  The rescaled partition function (\ref{topete})
is invariant, since the $-1$ change in the number $n^{\va (4)}_b-n^{\va (3)}_b$ is compensated by the 
remaining loop on the right diagram in Figure~{\ref{fig:9}} (contributing as $\tau^{+1}$).
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM4d42e} 
\includegraphics[width=4cm]{PM4d42f}}    
\caption{Ones all the internal cables have been eliminated (left diagram) a single closed loop
remains. Deforming the diagram and adding a redundant cable one arrives to the diagram on the right
where the $(4,2)$ move has been implemented. }\label{fig:9}
\end{figure}

\subsubsection{The $(3,3)$ move}

Invariance under the $(3,3)$ move follows immediately from applying the gauge-fixing identity
to two of the internal cables and then implementing (\ref{pito}) once to the cable-wire diagram corresponding
to the initial 4-simplex configuration described in section (\ref{Pach}) above. 
Figure~{\ref{femenino}} shows the result of these
operations. Once the three internal cables are removed one simply rearranges the internal wiring so that after
reinserting the three internal cables, using (\ref{cuatro}) and (\ref{pito})
in the inverse way, one obtains the correct final configuration. 
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{PM4d33a}}
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,
%\includegraphics[width=5cm]{PM4d33b}}
\caption{The initial three 4-simplex configuration (left). Internal cables are eliminated
using (\ref{cuatro}) and (\ref{pito}).}\label{femenino}
\end{figure}
In all this process the evaluation remains invariant, and, since 
the number $n^{\va (4)}_b-n^{\va (3)}_b$ does not change, the rescaled partition function (\ref{topete})
also remains invariant.
%\begin{figure}[h]\label{}
%\centerline{\hspace{0.5cm} 
%\includegraphics[width=5cm]{PM4d33c} 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
%\,\,\,\,\,\,\,\,\,\,\,\,\,\,
%\includegraphics[width=5cm]{PM4d33d}}
%\caption{Internal wires have been rearranged to obtain the final configuration in 
%the $(3,3)$ move (left). Internal cables are reinserted on the right using  (\ref{cuatro}) and (\ref{pito}). }
%\end{figure}

\subsection{General independence of ${\cal Z}_{BF}$ on the discretization of $\cal M$.}

We have shown the independence of the Partition function for BF theory on the
choice of simplicial decomposition (triangulation) of the manifold. As discussed in
Chapter (\ref{chp:bf}), this is not surprising since the theory we are dealing 
with contains only global degrees of freedom. Triangulation 
invariance appears then as a natural property of the path integration, since
global degrees of freedom can be appropriately captured 
with any triangulation. In particular, one would expect the partition function of BF theory to be
well defined for any discretization of $\cal M$, i.e., not necessarily a triangulation.
This expectation turns out to be true. In this section we sketch the proof of this assertion;
details of the rigorous proof can be found in  \cite{raf}.  
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{square} 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,
\includegraphics[width=5cm]{square1}}
\label{square}
\end{figure}  

\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{exa} 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\, 
\,\,\,\,\,\,\,\,\,\,\,\,\,\,
\includegraphics[width=5cm]{exa1}}
\label{exa}
\end{figure}

The notion of arbitrary discretization is realized by the notion of cellular decomposition of $\cal M$ so we  
we recall the definition of cellular complex (see  \cite{rour}) which we already mentioned in a different
context in Chapter {\ref{chp:bf}}. The basic element in the definition is that of ``cell''. 
A $0$-cell corresponds to a point, a $1$-cell to a closed interval, a $2$-cell to a polygon, etc. Any cell contains lower-dimensional cells referred to as faces. A cellular complex $\cal K$ is a collection of cells such that the intersection
of any two cells is in $\cal K$ and the face of any cell is again in $\cal K$.


The connection with previous results is given by the following proposition (see  \cite{rour}, page 16)

{\bf Proposition:} {\em A cellular complex $\cal K$ can be subdivided into a simplicial complex $\Delta_{\cal K}$ (triangulation) without introducing any new vertices.}
 
The independence of the BF path integral measure on arbitrary discretizations is stated in the following equation:
\begin{equation}
{\cal Z}_{BF}({\cal K})={\cal Z}_{BF}(\Delta_{\cal K}).
\end{equation}
In two dimensions this is a trivial consequence of equation (\ref{tdt}). The equivalence can be shown by
subdividing cell by cell in $\cal K$ and applying the gauge fixing
(\ref{tdt}) as is shown in Figures~{\ref{square}} and {\ref{exa}}. 
In higher dimensions the proof requires also equation (\ref{pito}), and the argument becomes
slightly more complicated. Here we give a schematic proof in three dimensions; the complete argument can be found in~\cite{raf}.


Think of an arbitrary polyhedron $\kappa$ with $N$ 
faces in three dimensions as part of the corresponding 
cellular complex ${\cal K}$. The corresponding dual cable-wire
diagram consists of $N$ external cables whose wires are appropriately connected
defining an $N$-valent dual vertex. Each cable contains as many wires as edges in the corresponding
face. In the simple case of a cube, the cable-wire diagram is given by a $6$-valent vertex of
4-valent cables (cables with four wires). In any subdivision of the polyhedron, which does not
include new vertices, faces will get triangulated so that the number of external cables in the 
corresponding cable-wire diagram dual to $\Delta_{\cal K}$ will be multiplied in each original face
by the corresponding number of triangles. Each cable is now 3-valent. 
Coming back to the example of the cube, going from ${\cal K}$
to $\Delta_{\cal K}$ each square face of the cube is replaced by two triangles, and the original 4-valent
cable is substituted by two 3-valent cables. There are $12$ external cables now. Inside our general
polyhedron new dual vertices and new faces appear after the subdivision. In the case of the cube the original
$6$-valent vertex splits into six interconnected 3-valent vertices 
(six tetrahedra are needed to triangulate the cube). Notice that according to the proposition
above no additional vertices are included in $\Delta_{\cal K}$; therefore, there will be new internal
faces in the polyhedron but they will not close forming a bubble. A moment of reflection shows 
that internal cables can be removed using the gauge-fixing equation (\ref{tres}) and the identity
(\ref{pito}) with no remaining closed-wire contribution. Thus, after this is done we end up with
a single dual vertex of 3-valent cables. In the case of the cube we end up with a single 12-valent
dual vertex in which all the cables are 3-valent. In order to conclude the proof we need
to reduce the number of cables and increment appropriately the corresponding valence to obtain our
original $N$-valent dual vertex. This can be done using the following identity
\begin{equation}\label{match}
\sum \limits_{k_1, \dots k_N} \Delta_{k_1} \dots  \Delta_{k_N}
\begin{array}{c} 
\includegraphics[width=4.cm]{match}\end{array} = \begin{array}{c} 
\includegraphics[width=1.6cm]{matcha}\end{array},
\end{equation}
which is a direct consequence of (\ref{martin}) above. From the definition of $\cal K$
we have that every face is shared by two polyhedra in $\cal K$. After the subdivision
of polyhedra each face gets triangulated as described above and new edges appear on the 
original face. There is a dual face around each such edge which corresponds to a 
closed-wire loop passing trough only two cables (remember that all the internal structure of the
cable-wire diagram corresponding to $\kappa$ has been reduced to a single vertex in the
interior). In the case of the cube this shown in Figure~{\ref{figu:11}}.
\begin{figure}[h]
\centerline{\hspace{0.5cm} 
\includegraphics[width=5cm]{front}} .
\label{figu:11}
\end{figure}
Therefore, we can use equation (\ref{match}) to reduce the multiple cables in the 
subdivision to obtain the single cable of the original cable-wire diagram of $\kappa$,
which completes the proof.        

